k-Color Multi-Robot Motion Planning

We present a simple and natural extension of the multi-robot motion planning problem where the robots are partitioned into groups (colors), such that in each group the robots are interchangeable. Every robot is no longer required to move to a specific target, but rather to some target placement that is assigned to its group. We call this problem k-color multi-robot motion planning and provide a sampling-based algorithm specifically designed for solving it. At the heart of the algorithm is a novel technique where the k-color problem is reduced to several discrete multi-robot motion planning problems. These reductions amplify basic samples into massive collections of free placements and paths for the robots. We demonstrate the performance of the algorithm by an implementation for the case of disc robots and polygonal robots translating in the plane. We show that the algorithm successfully and efficiently copes with a variety of challenging scenarios, involving many robots, while a simplified version of this algorithm, that can be viewed as an extension of a prevalent sampling-based algorithm for the k-color case, fails even on simple scenarios. Interestingly, our algorithm outperforms a well established implementation of PRM for the standard multi-robot problem, in which each robot has a distinct color.

==> sec_completeness.tex <==
\section{Toward Probabilistic Completeness of UPUMP}\label{sec:complete}\rsecafter
    We show that by making a simple assumption on the work of the connection generator, it can be proved that \algup is probabilistically complete. In order to do so we show that a simplified version of the \algup algorithm, called \algub, is probabilistically complete.
    Its  samples consist of pumped configurations of size $m$ (as opposed to size $n>m$ in Section~\ref{secUnlabeled}) which result in \emph{degenerate} pebble graphs where the number of vertices is equal to the number of pebbles. We prove the completeness of \algub by showing a reduction from the PRM algorithm for the fully-colored multi-robot motion planning problem. The completeness of \algup follows as a rather straightforward corollary.

    We stress that it still might be possible that \algup (and \algkp), in its original formulation, is probabilistically complete, and we hope that the efforts made in this section will ultimately assist in proving this.


    \subsection{The PRM Algorithm for the Fully-Colored Case}
        The PRM algorithm was initially designed to solve \sr motion planning problems. However, it can be used for solving the fully-colored multi-robot motion planning problem by considering the fleet of robots as one composite robot. We briefly describe the PRM algorithm for the fully-colored case. Recall that in the fully-colored problem, every robot $r_i$ is assigned with specific start and target positions $s_i,t_i$. For the purpose of the probabilistic completeness proof of \algup, we may assume that the robots are geometrically identical.

        Recall that the PRM algorithm for the \sr case consists of two main phases. In the preprocessing phase the algorithm samples a collection of valid \sr configurations. Then, for every sampled \sr configuration it finds its nearest neighbors and tries to connect it to the neighbors using the local planner. In the query phase, the start and target \sr configurations are connected to the constructed roadmap by considering connections to the nearest neighbors of the start and target, respectively.
        We intentionally avoid from referring to a specific neighbor finding technique since there are several methods that are suitable for this task. Our only requirement from the neighbor-finding technique is that it will lead to a probabilistically complete PRM algorithm.
        Such methods are described in the work of Karaman and Frazolli~\cite{kf-sbaomp11}, where the issue of completeness is discussed as well.

        In the case of the fully-colored multi-robot motion planning problem, every sample of the PRM consists of $m$ \sr configurations, one \sr configuration for every robot. In contrast with the unlabeled case, where every robot can be assigned with any \sr configuration, here every \sr configuration is associated with a specific robot. This is formalized in the following definition.

        \begin{definition}
            Let $C=\{c_1,\ldots,c_m\}$ be a configuration and let $\sigma$ be some permutation of $\{1,\ldots,m\}$. The \emph{ordered configuration} of $C$ for the permutation $\sigma$ is defined to be $\sigma(C)=(c_{\sigma(1)}, \ldots, c_{\sigma(m)})$.
        \end{definition}

        We denote by $\sigma_I$ the \emph{identity permutation}. In an ordered configuration $\sigma(C)$ a position of the robot $r_i$ is represented by $c_{\sigma(i)}$. Hence, the samples of the PRM algorithm for the fully-colored case are ordered configurations. For simplicity, we may assume that a configuration is sampled and a specific permutation $\sigma_{\text{PRM}}$ is assigned to it.
        A connection between two ordered configuration is achieved by applying the \emph{multi-robot local planner}. This component returns a set of $m$ paths between two ordered configuration (if they exist), one for each robot, such that they are all collision free, both with respect to the obstacles and with respect to the other robots.

        \begin{definition}
            Let $\sigma(C)=(c_1,\ldots,c_m), \sigma'(C')=(c'_1,\ldots,c'_m)$ be two ordered configurations.
            Denote by $\pi_i$ the path returned by the local planner (Section~\ref{subsec:constrion_pebble}) on the  input $c_i,c'_i$. Suppose that for every $i$, it holds that $\pi_i\neq \bot$, namely, the local planner successfully generated a path for the input $c_i,c'_i$. In addition, suppose that every pair of paths $\pi_i,\pi_j$ is collision free, i.e., for every $\theta\in [0,1]$, $r(\pi_i(\theta))\cap r(\pi_j(\theta))=\emptyset$ ,where $r(c)$, for $c\in \C$, represents the portion of the configuration space that is covered by the robot that is placed in $c$ (Section~\ref{secPreliminaries}). Then the \emph{multi-robot local planner} returns the set of paths $\{\pi_1,\ldots,\pi_m\}$. Otherwise, it returns $\bot$.
        \end{definition}

        If the multi-robot local planner successfully connects two ordered configurations, then an edge between them is added to the PRM roadmap. We summarize the steps of the PRM algorithm for the fully-colored problem. In the \emph{preprocessing} phase, PRM samples a collection of ordered configurations $\{\sigma_{\text{PRM}}(C_1),\ldots,\sigma_{\text{PRM}}(C_g)\}$.
        Then, for every sampled ordered configuration it finds a set of neighbors and attempts to connect them with the current sample. We refer to the roadmap that results from this process as the \emph{induced roadmap} of the samples $\sigma_{\text{PRM}}(C_1),\ldots,\sigma_{\text{PRM}}(C_g)$. In the \emph{query phase}, the PRM algorithm is given two ordered configurations $(s_1,\ldots,s_m),(t_1,\ldots,t_m)$, and attempts to connect them to the roadmap. The following theorem is a generalization of the completeness theorem for the \sr case~\cite{kf-sbaomp11}.

        \begin{theorem}\label{thm:prm_complete}
            Let $\{\U_1,\ldots,\U_m\}$ be a fully-colored problem where $\U_i=(r_i,s_i,t_i)$ for which there is a solution. Then there exist constants $a>0,g_0\in\dN$, such that a PRM algorithm with $g>g_0$ samples will find a solution with probability at least $1-e^{-ag}$.
        \end{theorem}

    \subsection{The UBASIC Algorithm}
        We present the \algub algorithm, which is a simplified version of the \algup algorithm.  The pseudo-code of \algub is identical to the one described for \algup in Section~\ref{secUnlabeled}. However, we set the number of vertices of the sampled pebble graphs to be $m$, i.e., we assign $n:=m$. This forces Algorithm~\ref{alg:geometric_graph} to generate configurations, instead of pumped configurations. In order to show that \algub is complete, we enforce an additional constraint on the connection generator. It is described next.

        Recall that the connection generator transforms the task of pathfinding between two pumped configurations to the problem of finding an independent set of size $m$, that represents a set of non-colliding paths, in the interference graph $\I$ (Section~\ref{sec:con}).  Currently, the independent sets in $\I$ are found using a greedy technique, which is not guaranteed to find a solution, even if one exists. We will introduce below an additional step to the connection generator that is guaranteed to find at least one solution, if exists. For now, we assume that the following assumption holds. We will discuss its impact on \algup later on.
        \begin{assumption}\label{assume:basic}%[Completeness of the Connection Generator]
            Let $C,C'$ be two configurations. Suppose that there exist two permutations, $\sigma,\sigma'$, for which the multi-robot local planner finds a path for the input $\sigma(C),\sigma'(C')$. Then, upon the application of the connection generator on the input $C,C'$, it returns at least one path $\pi_{C,C'}$, that is a solution to the unlabeled problem $\U'=(C,C')$.
        \end{assumption}

        Notice that we do not insist that the connection generator will return exactly the same path that was generated by the multi-robot local planner. The following observation shows that an unlabeled problem has a solution if and only if there exists a solution to some fully-colored problem from a family of problems. It is a crucial component in the probabilistic completeness proof of the \algub algorithm.

        \begin{observation}\label{obs}
            Let $\U=(R,S,T)$ be an unlabeled problem, where $R=\{r_1,\ldots,r_m\}, S=\{s_1,\ldots,s_m\}, T=\{t_1,\ldots,t_m\}$. There is a solution to $\U$ if and only if there exists a permutation $\sigma_T$, such that there is a solution to the fully-colored problem $\L=\{\U_1,\ldots, \U_m\}$, where $\U_i=(r_i,s_i,t'_i)$ and $\sigma_T(T)=(t'_1,\ldots,t'_m)$.
        \end{observation}

        \begin{lemma}\label{lem:equiv}
            Let $\C_1,\ldots,C_g$ be a collection of configurations sampled by {\algub} in the preprocessing stage. Denote by $G_{\text{PRM}}$ the PRM roadmap that is induced by the collection of PRM samples $\sigma_{\text{PRM}}(C_1),\ldots,\sigma_{\text{PRM}}(C_g)$. Suppose that there exists a permutation $\sigma_T$ for which the PRM algorithm, with the roadmap $G_{\text{PRM}}$, finds a solution for the query $\sigma_I(S),\sigma_T(T)$ (where $\sigma_I$ is the identity permutation). Then, \algub will successfully find a solution for the query $(S,T)$.
        \end{lemma}

        \begin{proof}
            Denote by $\sigma_I(S)=\sigma_I(C_0), \sigma_{\text{PRM}}(C_1),\ldots, \sigma_{\text{PRM}}(C_{\ell-1}), \sigma_T(C_{\ell})=\sigma_T(T)$, the path that was found by the PRM roadmap $G_{\text{PRM}}$ after connecting the query $\sigma_I(S), \sigma_T(T)$. Thus, the multi-robot local planner successfully connected every pair of consecutive ordered configurations $\sigma_{\text{PRM}}(C_i),\sigma_{\text{PRM}}(C_{i+1})$ along the path (the same applies to the ends of the path). By Assumption~\ref{assume:basic}, we deduce that the connection generator successfully connects $C_i,C_{i+1}$. Thus, $C_i,C_{i+1}$ are connected in the roadmap $\H$ in the \algub algorithm.\qed
        \end{proof}

        Using this connection between PRM and UBASIC we show that the latter is probabilistically complete.

        \begin{theorem}\label{thm:complete_upump}
            Let $\U=(R,S,T)$ be an unlabeled problem for which there is a solution. Then there exist constants $a>0,g_0\in\dN$, such that the \algub algorithm with $g>g_0$ samples will find a solution with probability at least $1-e^{-ag}$.
        \end{theorem}
        \begin{proof}
            By Observation~\ref{obs}, there exists a permutation $\sigma_T$ for which there is a solution to the fully colored problem $\L=\{\U_1,\ldots, \U_m\}$, where $\U_i=(r_i,s_i,t'_i)$ and $\sigma_T(T)=(t'_1,\ldots,t'_m)$. Let $C_1,\ldots, C_g$ be the collection of the $g$ configurations sampled by \algub. By Theorem~\ref{thm:prm_complete}, the PRM algorithm, with the roadmap induced by the samples $\sigma_{\text{PRM}}(C_1),\ldots,\sigma_{\text{PRM}}(C_g)$, will find a solution for the query $\sigma_I(S),\sigma_T(T)$, with probability at least $1-e^{-ag}$. If the latter occurs, then by Lemma~\ref{lem:equiv}, \algub finds a solution as well. Thus, \algup finds a solution with probability at least $1-e^{-ag}$.\qed
        \end{proof}

        \noindent\textbf{Remark.} We mention that for the purpose of experiments (Section~\ref{sec:results}) we use a more efficient version of UPUMP (and KPUMP) that similarly to the PRM connects only nearby samples, where distance between configuration-samples is measured using Hausdorff distance.

    \subsection{Extending Completeness to UPUMP}
        We force \algup to generate a roadmap that simulates a run of the \algub, by modifying Assumption~\ref{assume:basic}. Recall, that in the \algup algorithm, the connection generator is applied on pumped configurations (and not configurations, as in \algub).

        Let $V=\{v_1,\ldots,v_n\}$ be a pumped configuration. Denote by $V(m)$ the configuration that consists the first $m$ elements of $V$.
        \begin{assumption}\label{assume:pump}%[Completeness of the Connection Generator]
            Let $V,V'$ be two pumped configurations. Suppose that there exist two permutations, $\sigma,\sigma'$, for which the multi-robot local planner finds a path for the input $\sigma(V(m)),\sigma'((V'(m))$. Then, upon the application of the connection generator on the input pumped configurations $V,V'$, it must return at least one path $\pi_{V,V'}$, that is a solution to the unlabeled problem $\U'=(V,V')$.
        \end{assumption}

        Under this Assumption~\ref{assume:pump}, we extend Lemma~\ref{lem:equiv} for the \algup algorithm.

        \begin{lemma}\label{lem:equiv}
            Let $G_1,\ldots,G_g$ be a collection of pebble graphs sampled by {\algup} in the preprocessing stage, where $G_i=(V_i,E_i)$, and $V_i$ is a pumped configuration. Denote by $G_{\text{PRM}}$ the PRM roadmap that is induced by the collection of PRM samples $\sigma_{\text{PRM}}(V_1(m)),\ldots,\sigma_{\text{PRM}}(V_g(m))$. Suppose that there exists a permutation $\sigma_T$ for which the PRM algorithm, with the roadmap $G_{\text{PRM}}$, finds a solution for the query $\sigma_I(S),\sigma_T(T)$. Then, \algup will successfully find a solution for the query $(S,T)$.
        \end{lemma}

        The proof is trivial, and hence omitted. The following corollary immediately follows.

        \begin{corollary}
            Let $\U=(R,S,T)$ be an unlabeled problem for which there is a solution. Then there exist constants $a>0,g_0\in\dN$, such that the \algup algorithm with $g>g_0$ samples of pebble graphs will find a solution with probability at least $1-e^{-ag}$.
        \end{corollary}

    \subsection{Reinforcing the Connection Generator}
        As mentioned earlier, in its current state (as described in Section~\ref{sec:con}) the connection generator does not fulfil the requirement of Assumption~\ref{assume:basic}. Thus, a modification of the component is required if we wish guarantee the correctness of Theorem~\ref{thm:complete_upump}.

        We describe a simple alternative implementation of the connection generator component that is based on \emph{integer programming} (IP) and guarantees to find a connection if one exists, thus fulfilling Assumption~\ref{assume:basic}.

        Recall that in \algub the connection generator is given two configurations $V=\{v_1,\ldots,v_m\}$, $V'=\{v'_1,\ldots,v'_m\}$. In addition, recall that $\R=\{(v,v')|v\in V,v'\in V',\;\pi_{v,v'}\neq\bot\}$ is the set of all pairs of elements from $V,V'$ for which the local planner successfully generated a path. To every pair $(v,v')\in\R$ we assign the boolean variable $x_{v,v'}\in\{0,1\}$ that indicates whether the respective path is selected for the connection. Our goal is to find $m$ non-interfering pairs. This results in the following two constraints.
        \begin{enumerate}
            \item If $(v,v'),(u,u')\in \R$ \emph{interfere} then $x_{v,v'}+ x_{u,u'}\leq 1$.
            \item $\sum_{(v,v')\in \R}x_{v,v'}=m$.
        \end{enumerate}

        We mention that although the problem of integer programming is known to be NP-hard~\cite{p-cc94}, in practice these problems can be solved efficiently using various software packages, e.g.,~\cite{cplex07}.






==> sec_completeness2.tex <==
\section{OLD - Completeness of \Balgup}\label{sec:complete}\rsecafter
    Using a few modification to the original algorithm, presented in Section~\ref{secUnlabeled}, we show that \algup is probabilistically complete. In order to do so we show that a simplified version of the \algup algorithm, called \algub, is probabilistically complete.
    This algorithm does not allow the robots to move as pebbles. Its  samples consist of pumped configurations of size $m$ (as opposed to size $n>m$ in Section~\ref{secUnlabeled}) which result in \emph{degenerate} pebble graphs where the number of vertices is equal to the number of pebbles. We prove that completeness of \algub by simulating using it the PRM algorithm for the case of a fully-colored multi-robot motion planning problem. We later show how this can be extended to \algup.

    \subsection{The PRM Algorithm for the Fully-Colored Case}
        The PRM algorithm was initially designed to solve \sr motion planning problems. However, it can be used for solving fully-colored problems by considering the fleet of robots as one composite robot. We briefly describe the PRM algorithm for the fully-colored case.

        Recall that in the fully-colored multi-robot motion planning problem, every robot $r_i$ is assigned with specific start and target positions $s_i,t_i$. Since we will use fully-colored planner to solve the unlabeled problem we may assume that all the robots are geometrically identical.

        Recall that the PRM algorithm for the \sr consists of two main phases. In the preprocessing phase the algorithm samples a collection of valid \sr configurations. Then, for every sampled \sr configuration it finds its $k$ nearest neighbors and tries to connect it to the neighbors using the local planner. In the query phase, the start and target \sr configurations are connected to the this roadmap by considering connections to $k$ nearest neighbors of start and target.

        In the colored case, every sample of the PRM consists of $m$ \sr configurations, one \sr for every robot. In contrast with the unlabeled case, where every robot can be assigned with any \sr configuration, here every \sr configuration is associated with a specific robot. This is formally defined in the following definition.

        \begin{definition}
            Let $C=\{c_1,\ldots,c_m\}$ be a configuration and let $\sigma$ be some permutation of $\{1,\ldots,m\}$. The \emph{ordered configuration} of $C$ for the permutation $\sigma$ is defined to be $\sigma(C)=(c_{\sigma(1)}, \ldots, c_{\sigma(m)})$.
        \end{definition}

        In an ordered configuration $\sigma(C)$, as defined above, a position of the robot $r_i$ is represented by $c_{\sigma(i)}$. Hence, the samples of the PRM algorithm for the fully-colored case are ordered configurations. For simplicity, we may assume that a configuration is sampled and a specific permutation $\sigma$ is assigned to it.
        A connection between two ordered configuration is achieved by applying the \emph{multi-robot local planner}.

        \begin{definition}
            Let $\sigma(C)=(c_1,\ldots,c_m), \sigma(C')=(c'_1,\ldots,c'_m)$ be two ordered configurations.
            Denote by $\pi_i$ the path that is returned by the local planner (Section~\ref{subsec:constrion_pebble}) on the  input $c_i,c'_i$. Suppose that for every $i$ $\pi_i\neq \bot$, namely, the local planner successfully generated a path for the input $c_i,c'_i$. In addition, suppose that every pair of paths $\pi_i,\pi_j$ is collision free, i.e., for every $\theta\in [0,1]$, $R(\pi_i(\theta))\cap R(\pi_j(\theta))=\emptyset$. Then the \emph{multi-robot local planner} returns the set of paths $\{\pi_1,\ldots,\pi_m\}$. Otherwise, it returns $\bot$.
        \end{definition}

        If the multi-robot local planner successfully connects two ordered configurations, then an edge between them is added to the PRM roadmap. The following is a generalization of the completeness theorem for the \sr case.

        \begin{theorem}
            Let $\{\U_1,\ldots,\U_m\}$ be a fully-colored problem where $\U_i=(r_i,s_i,t_i)$ for which there is a solution. Then there exist constant $a>0,g_0\in\dN$, such that a PRM algorithm with $g>g_0$ samples will find a solution with probability at least $1-e^{-ag}$.
        \end{theorem}

        A simple modification to the PRM algorithm will yield a probabilistically complete algorithm for the unlabeled problem. Let $\U=(R,S,T)$ be our input unlabeled problem. If this problem has a solution then there exist two permutations $\sigma_S,\sigma_T$ such that the fully-colored problem $\{\U_1,\ldots,\U_m\}$ has a solution, where $\U_i=(r_i,s'_i,t'_i)$ and $\sigma_S(S)=(s'_1,\ldots,s'_m), \sigma_T(T)=(t'_1,\ldots,t'_m)$. Thus, given a sufficient amount of samples $g$ of the PRM algorithm, and the correct permutations $\sigma_S,\sigma_T$, a solution can be found. Unfortunately, it is not clear how the permutations can be determined beforehand. Notice that the start permutation $\sigma_S$ determines $\sigma_T$. Thus, we can fix $\sigma_S$ and need to find a ``feasible'' $\sigma_T$.

        The PRM-based algorithm for the unlabeled problem, called uPRM, works in the following manner. The preprocessing phase of this algorithm is identical to the same stage in the original PRM algorithm. Recall that in the preprocessing stage two ordered configurations were connected to the roadmap by finding the nearest neighbors in the roadmap of every ordered configuration. In the case of uPRM, we will try to connect many more ordered configurations to the roadmap: First, we connect $\sigma_S(S)$. Then, for every permutation $\sigma'$ we try to connect the ordered configuration $\sigma'(T)$. Finally, if for one of the permutations $\sigma'(T)$ lies in the same component of the PRM roadmap as $\sigma_S(S)$ the algorithm returns the respective path and terminates. We stress that the construction of the roadmap is performed once, as in the PRM algorithm.

    \subsection{The \Balgub Algorithm}
        We first describe the preprocessing stage of the \algub algorithm, which resembles to the same step in the \algup (Algorithm~\ref{alg:preprocess}), with two small modifications. As mentioned earlier, every sampled pebble graph has $m$ vertices (where the $m$ is the actual number of robots), instead of $n$ in the original algorithm. Consequently, this forces Algorithm~\ref{alg:geometric_graph} to generate configurations, instead of pumped configurations.

        In addition, we replace the CONNECT routine (Algorithm~\ref{alg:connect}) with CONNECT* (Algorithm~\ref{alg:connect_star}) that applies the multi-robot local planner, before attempting to connect the two pebble graphs with a connection generator. Notice, that in the case of the \algub algorithm a single successful connection between two pebble graphs suffices since the pebble graphs are in fact configurations. Thus, we can set $q=1$, where $q$ is the number of desired connection produced by the connection generator.

        \begin{algorithm}[b]
            \caption{CONNECT*($G=(V,E),G'=(V',E'),\H=(\V,\E),q$)}
            \label{alg:connect_star}
            \begin{algorithmic}[1]
                \STATE  $\Pi \leftarrow\text{MULTI\_ROBOT\_LP} (\sigma(V),\sigma(V'))$
                \IF     {$\Pi\neq \bot$}
                    \STATE $\E\leftarrow \E\cup\{(V,V')\}$
                \ENDIF
                \STATE CONNECT$(G,G',\H,q)$
            \end{algorithmic}
        \end{algorithm}

        \begin{comment}
        The second modification is the following assumption that is enforced on the connection generator (Section~\ref{sec:con}).

        \begin{assumption}\label{assumption:congen}
            Let $G=(V,E),G'=(V',E)$ be two geometric graphs such that $V=(c_1,\ldots,c_m),V'=(c'_1,\ldots,c'_m)$. Let $\sigma$ be the permutation used by the PRM algorithm.

            Then, the connection generator, given the input $G,G'$, returns the path $\pi$ that is a solution to the fully-colored problem $\{\U_1,\ldots,\U_m\}$ $\U_i=(r_i,v^*_i,{v'}^*_i)$ and $\sigma(V)=(v^*_1,\ldots,v^*_m), \sigma(V')=({v'}^*_1,\ldots,{v'}^*_m)$.
        \end{assumption}


        Under this assumption, the roadmap $\H$ that is constructed by \algub contains information regarding paths that would have been found by the PRM algorithm.
        \end{comment}

        \begin{definition}
            Let $\G=\{G_1,\ldots,G_g\}$ be the set of pebble graphs sampled by \algub, where $G_i=(V_i,E_i)$ and $V_i$ is a configuration. The \emph{PRM roadmap induced by \algub} is defined to be the PRM roadmap of the samples $\sigma(V_1),\ldots,\sigma(V_g)$.
        \end{definition}

        \begin{lemma}
            Let $C,C'$ be two vertices of the roadmap $\H$. If $\sigma(C),\sigma(C')$ are connected in the induced PRM roadmap, then $C,C'$ are connected in $\H$.
        \end{lemma}

        \begin{proof}
            Let $\sigma(C)=\sigma(C_1), \ldots, \sigma(C_{\ell})=\sigma(C')$ be the vertex path in the PRM roadmap. Then, for every $\sigma(C_i), \sigma(C_{i+1})$ the multi-robot local planner successfully connected the two order configurations. Therefore, the CONNECT* routine will add an edge in $\E$ between $C_i$ and $C_{i+1}$.
        \end{proof}

        In order to show that \algup has a success rate that is as high as uPRM, for the same number of samples $g$, we will force \algup to perform the query stage of uPRM and only then perform the QUERY routine of \algup (Algorithm~\ref{alg:query}). Specifically, the query stage of uPRM will be performed on the induced PRM roadmap of \algup.

        \begin{corollary}
            Let $\U=(R,S,T)$ be an unlabeled problem for which there is a solution. Then there exist constant $a>0,g_0\in\dN$, such that the \algub algorithm with $g>g_0$ samples of configurations will find a solution with probability at least $1-e^{-ag}$.
        \end{corollary}

    \subsection{Extending Completeness to \Balgup}
        No special modification to the original algorithm, beyond the ones that were just presented, are required. Recall, that in the case of \algup we sample pumped configurations. Thus, we need to specify how to convert the samples of \algup to samples of uPRM.

        \begin{definition}
            Let $V={c_1,\ldots,c_n}$ be a pumped configuration. Let $\sigma$ be a permutation of $m$ elements. We define $\sigma(V)=\sigma(C)$, where $C\subset V$ is a configuration such that $C=\{c_1,\ldots,c_m\}$.
        \end{definition}

        The following corollary immediately follows.

        \begin{corollary}
            Let $\U=(R,S,T)$ be an unlabeled problem for which there is a solution. Then there exist constant $a>0,g_0\in\dN$, such that the \algup algorithm with $g>g_0$ samples of pebble graphs will find a solution with probability at least $1-e^{-ag}$.
        \end{corollary}


==> sec_completeness_old.tex <==
\section{Probabilistic Completeness of \Balgup} \label{sec:completenss}\rsecafter 

    \subsection{PRM Variant for the Unlabeled Problem}
    \begin{definition}
        Let $C=\{c_1,\ldots,c_m\}$ be a configuration and let $\sigma$ be a permutation of $m$ elements. The \emph{ordered configuration} of $C$ for the permutation $\sigma$ is defined to be $C_{\sigma}=\left(c_{\sigma(1)},\ldots, c_{\sigma(m)}\right)$.
    \end{definition}
    
    \begin{algorithm}[H]
            \caption{PRM\_PREPROCESS}
            \label{alg:prm_preprocess}
            \begin{algorithmic}[1]
                \STATE  $\dV\leftarrow\emptyset,\dE\leftarrow\emptyset$
                \WHILE  {$|\dV|\neq g$}
                    \STATE  $C=\text{PUMPED\_CONFIGURATION}(m)$
                    \STATE  $\dV\leftarrow\dV\cup\{C_{\sigma^*}\}$
                \ENDWHILE
                \FORALL    {$C_{\sigma^*}\in\dV$}
                    \STATE  $U\leftarrow \text{NEAR}(\dV,C_{\sigma^*})$
                    \FORALL {$C'_{\sigma^*}\in\dV, C'_{\sigma^*}\neq C_{\sigma^*}$}
                        \IF     {$\text{MULTI\_LP}(C_{\sigma^*},C'_{\sigma^*})\neq \bot$}
                            \STATE $\dE\leftarrow\dE\cup\{(C_{\sigma^*},C'_{\sigma^*})\}$
                        \ENDIF
                    \ENDFOR
                \ENDFOR
            \end{algorithmic}
        \end{algorithm}
        
        
    \begin{algorithm}[H]
    \caption{MULTI\_LP($C_{\sigma^*}=(c_1,\ldots,c_m), C'_{\sigma^*}=(c'_1,\ldots,c'_m)$)}
    \label{alg:multi_lp}
        \begin{algorithmic}[1]
            \STATE  $\Pi\leftarrow \emptyset$
            \FOR    {$i=1\to m$}
                \STATE  $\pi\leftarrow \text{LOCAL\_PLANNER}(c_i,c'_i)$
                \IF     {$\pi\neq \bot$}
                    \STATE $\Pi\leftarrow \Pi\cup\{\pi\}$
                \ELSE
                    \RETURN $\bot$
                \ENDIF
            \ENDFOR
            \RETURN $\Pi$
        \end{algorithmic}
    \end{algorithm}
    
    \begin{algorithm}[H]
    \caption{PRM\_QUERY}
    \label{alg:prm_query}
        \begin{algorithmic}[1]
            \STATE  $\Pi\leftarrow \emptyset$
            \FOR    {$i=1\to m$}
                \STATE  $\pi\leftarrow \text{LOCAL\_PLANNER}(c_i,c'_i)$
                \IF     {$\pi\neq \bot$}
                    \STATE $\Pi\leftarrow \Pi\cup\{\pi\}$
                \ELSE
                    \RETURN $\bot$
                \ENDIF
            \ENDFOR
            \RETURN $\Pi$
        \end{algorithmic}
    \end{algorithm}

==> sec_congen.tex <==
\section{Algorithm for the $k$-Color Connection Generator}
    In this section we describe an algorithm for the $k$-color connection generator component, used by \algkp. The algorithm has a preprocessing phase where single-robot paths are produced and the interactions between them are encoded in a graph. In the query phase subsets of the vertices of this graph are selected where each subset is transformed into a path from one composite configuration in the first cluster to a composite configuration in the second cluster.

    Let $\L=\{\U_i=(R_i,S_i,T_i)\}_{i=1}^k$ be a $k$-color problem where $|R_i|=m_i$. Let $\dM=\{m_1,\ldots,m_k\}$. In addition, let $\C_{\dG},\C_{\dG'}$ be two clusters that resulted from the pumped configurations $\dV=\{V_1,\ldots,V_k\},\dV'=\{V'_1,\ldots,V'_k\}$, respectively. Recall that the task of the connection generator is to find paths from composite configurations in $\C_{\dG}$ to composite configurations in $\C_{\dG'}$.  Throughout this section we will use the \emph{single-robot local planner} mechanism that given two single-robot configuration $c,c'$ for the robot $r$ will generate a path $\pi_{c,c'}$ from $c$ to $c'$. Notice that this mechanism does not consider the positions of other robots, in contrast to the edge planner.

    The algorithm transforms the problem of finding paths between clusters into a problem of finding a special case of an \emph{independent set} (IS) in an undirected graph. For every unlabeled problem $\U_i$ we generate a set of pairs $\mathcal{E}_i=\{(v,v')|v\in V_i,v'\in V'_i,\;\pi_{v,v'}\neq\bot\}$ where $\pi_{v,v'}$ is a path for a robot $r\in R_i$. Namely, these are pairs of elements from $V_i,V'_i$ for which the single-robot local planner successfully generated a path.

    For any $i,j$ we say that two pairs $(v,v')\in\E_i, (u,u')\in\E_j$ \emph{interfere} if there exists $\theta\in[0,1]$ such that robot $r\in R_i$ placed in $\pi_{v,v'}(\theta)$ collides with a robot $r'\in R_j$ placed in $\pi_{u,u'}(\theta)$. Notice that every two pairs $(v,v'),(u,u')\in\E_i$, such that $v=u$ or $v'=u'$, interfere by definition. We construct the \emph{interference graph} $\I$ whose vertices are the elements of $\bigcup_{i=1}^k \E_i$. We draw an edge between every two vertices of $\I$, $(v,v'),(u,u')$ that interfere.

    \begin{definition}[$\dM$-IS]
        Let $\S$ be an independent set of the vertices of $\I$. $\S$ is an $\dM$-IS if for every $1\leq i\leq k$ it contains exactly $m_i$ elements from $\E_i$.
    \end{definition}

    Given $\S$ that is $\dM$-IS we construct a $k$-color path. Let $\E'_i=S\cap \E_i = \{(u_1,u'_1),\ldots,(u_{m_i},u'_{m_i})\}$ where for every $1\leq j\leq m_i$, $u_j\in V_i$ and $u_j'\in V'_i $. We generate an unlabeled path $\pi_{\U'_i}$ for the unlabeled problem $\U'_i=(R_i,S'_i,T'_i)$ where $S'_i=\{u_1,\ldots,u_{m_i}\},T'_i=\{u'_1,\ldots,u'_{m_i}\}$. The unlabeled path is defined as the combination of the single-robot paths represented by the elements of $\mathcal{E}'_i$ . Namely, for every $\theta\in [0,1]$, $\pi_{\U'_i}(\theta)=\{\pi_{u_1,u'_1}(\theta),\ldots,\pi_{u_{m_i},u'_{m_i}}(\theta)\}$. As these paths form an independent set in $\mathcal{I}$ the robots of $R_i$ moving along $\mathcal{U}_i$ will not collide. Similarly, we define the path for the $k$-color problem to be $\pi_{\L'}(\theta)= \{\pi_{\U'_1}(\theta),\ldots ,\pi_{\U'_k}(\theta)\}$ for every $\theta\in [0,1]$.

    This is the algorithm that we implemented and with which the results reported in the experimental section of the main paper were obtained.


==> sec_congen_short.tex <==
\vspace{-10pt}
\section{The Connection Generator}\label{sec:con}\rsecafter
    We describe an algorithm for the connection generator component (CONGEN), used by \algup. Recall that the \congen is given two pumped configurations $V,V'$ and an integer $q$ that represents the number of desired connections. Throughout this section we will use the \emph{local planner} mechanism, that was used in the implementation of the \emph{edge planner} (Section~\ref{subsec:constrion_pebble}). Recall that given two single-robot configurations $v,v'\in \F$ the local planner attempts to construct a path $\pi_{v,v'}$ for a robot $r\in R$ from $v$ to~$v'$.

    The algorithm transforms the problem of finding paths between pumped configurations into the problem of finding an \emph{independent set} in an undirected graph. We generate the set of pairs $\R=\{(v,v')|v\in V,v'\in V',\;\pi_{v,v'}\neq\bot\}$. Namely, these are pairs of elements from $V,V'$ for which the local planner successfully generated a path. We say that two pairs $(v,v'),(u,u')\in\R$ \emph{interfere} if there exists $\theta\in[0,1]$ such that a robot $r\in R$ placed in $\pi_{v,v'}(\theta)$ collides with another robot $r'\in R$ placed in $\pi_{u,u'}(\theta)$. Notice that every two pairs $(v,v'),(u,u')\in\R$, such that $v=u$ or $v'=u'$, interfere by definition. We construct the \emph{interference graph} $\I$ whose vertices are the elements of $\R$, i.e., every vertex of $\I$ represents a path. We connect a pair of vertices of $\I$ by an edge if they interfere.

    Notice that by definition, every independent set of size $m$ of the vertices of $\I$ represents a collection of $m$ non-colliding single-robot paths. Note that the problem of finding an independent set is known to be NP-Hard~\cite{p-cc94}.

    We devised the following heuristic to find several independent sets: vertices of the graph are examined one by one, when the order is determined by a random permutation of the vertices. A new vertex is added to the set only if it is not connected to other vertices that are already in the set.\vspace{5pt}

    \noindent\textbf{Remark.} We concede that our approach to finding an independent set is not guaranteed to find a solution. This may impede attempts to prove the completeness of the \algup algorithm. We address this issue in Section~\ref{sec:complete} and state the modification that could lead to a probabilistic completeness proof of \algup.


==> sec_discussion.tex <==
\section{Discussion and Further Work}\label{sec:discussion}\rsecafter
    In this section we discuss the various properties of the \algkp algorithm and novelties it encompasses, as well as directions for future research.

    %\noindent\textbf{Shortcomings of the Composite Robot Approach.}
    \subsection{Shortcomings of the Composite Robot Approach}
    The traditional composite robot approach to the \mr problem treats the group of robots as one composite robot whose configuration space is the Cartesian product of the configuration spaces of the individual robots.
    With this approach, single-robot tools, such as \sbs algorithms, can be used to solve \mr problems.
    For instance, this technique is used in the software packages OOPSMP and OMPL~\cite{ompl,oopsmp} where PRM is applied to the fully-colored problem, and in the \algkb algorithm discussed above.
    Paths generated by this approach usually force the robots to move simultaneously from one placement to the other, where none of the robots remains in the same position while the others are moving.
    Although simultaneous movement of the robots is necessary in some cases, algorithms that consider only this type of movement may not fully exploit the properties of the \mr motion planning problem, and thus suffer from poor running time.

    Given collision-free placements for all the robots it is usually possible to move some of the robots to different placements without altering the placements of the rest of the robots, i.e., those robots remain still.
    For instance, consider a configuration $C=\{c_1,\ldots,c_m\}$ for some unlabeled problem $\U$.
    Unless the workspace is extremely tight, another configuration $C'$ can be derived from $C$ where only $c_1$ is moved to $c'_1$.
    Moreover, connecting two such configurations by a path requires only a \sr collision-free path for which the moving robot does not collide with the other robots placed in $c_2,\ldots,c_m$.
    In contrast, the connection of two ``unrelated'' configurations by a path imposes much harder constraints---$m$ single-robot collision-free paths have to be created and in addition, robots moving along those paths must not collide with each other.

    \algkp utilizes this observation by restricting the movements of the robots along certain path sections---induced by pebble problems---to motions of individual robots. We emphasize that \algkp does not preclude simultaneous movements of robots when necessary, specifically on path sections where the robots move from one pebble graph to the other along paths generated by the connection generator. We mention that sequential movements may result in longer paths, but this is a price that we are willing to pay, as we are able to cope with large groups of robots.

%    \noindent\textbf{Amplification of Samples.}
    \subsection{Amplification of Samples}
    Pumped configurations that are sampled by \algkp, and the resulting pebble graphs, are fairly simple structures which require only little effort to generate.
    Yet, using the transformation to pebble problem, these samples are amplified to describe not only placements and paths for single robots, but also to represent an incredible amount of paths and positions for all the robots in a given problem.
    However, this information is not represented explicitly and only little storage space is required to represent a pebble graph. In addition, a small number of configurations must be stored.
    Specifically, these are \confs through which the pebble graphs connects to other graphs.
    Such \confs are selected by the \emph{connection generator}.
    Similarly, this component does not require an explicit representation of all the configurations represented by the pebble graph.
    Furthermore, continuing the theme presented here that one action leads to a large number of outcomes, namely, a sample of a pumped configuration results in many configurations, a path generated by a connection generator not only connects two configurations from the two pebble graphs, but also a large number of \confs from them, which are not necessarily directly connected.
    Thus, these properties enable \algkp to generate a variety of configurations and motions of the robots, using only few samples. To reproduce this variety by \algkb one must generate far more samples.

    An additional advantage of the use of pebble graphs lies in the fact that they can be connected more easily than two configurations, when a powerful component as the connection generator is at hand.
    Using this component, \algkp succeeds in solving difficult scenarios even when the generated pebble graphs suffer from low connectivity, as in scenarios (c) and (d).%\vspace{5pt}

    \subsection{Further Work}
    Our immediate future goal is to investigate the completeness of the original formulation of the algorithm, i.e., using the connection generator algorithm that appears in Section~\ref{secUnlabeled}. In addition, it would be interesting to apply KPUMP to problems that involve more complex robots (e.g., rotating and translating polygons in the plane, multi-link robots). Additionally, it would be advantageous to reduce the number of parameters on which the algorithm relies.

    The experiments carried in this work suggest that the $k$-color problem, for various values of $k$, is less challenging than a fully-colored problem (with the same number of robots). Hence, it is an interesting problem to investigate the computational complexity of the unlabeled and $k$-color problems.

    There are many interesting variants of multi-robot motion planning, where we believe our approach can be applied. Some interesting applications will necessitate adaptation of KPUMP as described here since these problems have additional ingredients, such as distributed behaviour.   We mention the problem of flocking~\cite{r-fhs87,bla-rbf02} and crowd simulation~\cite{blm-rvo,tcp-cc06} that have some relation to the problem of multi-robot motion planning.

==> sec_experiments.tex <==
\begin{figure*}[!htp]
    \rimgbefore
            \centering
            \setlength{\tabcolsep}{3pt}
            \begin{tabular}{ccc}
                \subfloat{\includegraphics[width=0.3\columnwidth]{fig/scene_unlabeled25_path.pdf}} &
                \subfloat{\includegraphics[width=0.3\columnwidth]{fig/scene_2color_path.pdf}} &
                \subfloat{\includegraphics[width=0.3\columnwidth]{fig/scene_fully_decoupled_path.pdf}}\\
                (a) Unlabeled&
                (b) $2$-Color&
                (c) Fully-Colored: Decoupled
            \end{tabular}
            \begin{tabular}{cc}
                \subfloat{\includegraphics[width=0.4\columnwidth]{fig/scene_fully_coupled5_path.pdf}} &
                \subfloat{\includegraphics[width=0.3\columnwidth]{fig/scene_4color_path.pdf}}\\
                (d) Fully-Colored: Coupled&
                (e) $4$-Color
            \end{tabular}
            \vspace{-5pt}
            \caption{Scenarios for the case of disc robots. Start positions of the robots are indicated by discs while target positions are illustrated as circles in respective colors (unless otherwise indicated). (a) Unlabeled scene with twenty five robots. (b) $2$-Color scene; the two groups are required to switch positions. (c) Fully-colored scene with eight robots. (d) Fully-colored scene with five robots. (e) $4$-Color scene; every group has to move in a clockwise manner to the next room. }
            \label{fig:scenarios} %\vspace{-25pt}
        \end{figure*}
\section{Experimental Results}\label{sec:results}\rsecafter
    We describe experimental results for the case of disc robots and polygonal robots translating amidst polygonal obstacles in the plane. We show results for several challenging scenarios and compare the performance of \algkp with two other \sbs algorithms. Specifically we compare \algkp with the PRM implementation of the OOPSMP package~\cite{oopsmp} on inputs of the fully-colored problem. For other inputs we use a basic \sbs algorithm for the $k$-color problem called \algkb, described later on.

    \algkp was implemented in C++ using CGAL Arrangements~\cite{fhw-ca} and the Boost Graph Library (BGL)~\cite{sll-bgl}. The code was tested on a PC with Intel i7-2600 3.40GHz processor with 8GB of memory, running a Windows 7 64-bit OS. For the implementation of the \emph{local planner} a straight-line connection strategy was used. This strategy attempts to move the robot along a straight line drawn between two positions.\vspace{5pt}

    \noindent\textbf{Parameters of \Balgkp.}
    The algorithm has three parameters that affect its performance: $g$ describes the number of the sampled pebble graphs in the \algup algorithm, or the number of composite pebble graphs in \algkp; $q$ is the number of connections produced by the connection generator between two samples; $\mu$ is the maximal number of \sr configurations that one sample comprises, i.e., for every sampled pumped configuration $\dV=\{V_1,\ldots,V_k\}$ it holds that $\sum |V_i|\leq \mu$.
    The value of the latter parameter depends on the input problem.
    For unlabeled problems, increasing $\mu$ results in increased connectivity of the resulting pebble graphs. Thus, it will be beneficial that the pumped configurations will be as large as possible (limited by the topology of the scenario).
    On the other hand, in $k$-colored problems where $k>1$ the value $\mu$ has to be set more carefully as an excessively high value of $\mu$ will reduce the connectivity of the pebble graphs.
    This stems from the fact that a \sr path produced by the edge planner has to avoid collision with robots from other groups. Consequently, as the value of $\mu$ grows it becomes harder to connect \sr configurations using an edge planner.
    \begin{table}%{r}{0.5\textwidth}
        %\vspace{-10pt}
            \centering
            \caption{\label{table:res} Results for selected scenarios. Scenarios of polygonal robots are indicated by (*).}
                \begin{tabular}{|c||c|c|c||c|c|c||c|}
                    \hline
                    \multicolumn{1}{|c||}{\multirow{2}{*}{ }} & \multicolumn{3}{c||}{Properties} & \multicolumn{3}{c||}{Parameters} & \multicolumn{1}{c|}{\multirow{2}{*}{Time}} \\
                    \cline{2-7}
                     &$k$&$m$&$M$&$g$&$q$&$\mu$&\\
                    \hline
                    \hline
                    (a)&1&25&25&2&5000&150&23\\
                    (b)&2&8&16&50&1000&40&20\\
                    (c)&8&1&8&100&150&32&213\\
                    (d)&5&1&5&50&100&25&2\\
                    (e)&4&3&12&40&250&28&33\\
                    \hline
                    (a*)&2&4&8&20&250&16&13\\
                    (b*)&2&5&10&30&500&20&54\\
                    (c*)&3&1,4&6&30&250&20&11\\
                    (d*)&3&4&12&40&250&30&450\\
                    \hline
                \end{tabular}
                \label{table:res}
                \vspace{-15pt}
        \end{table}

        \begin{figure*}[!hbp]
    \rimgbefore
            \centering
            \setlength{\tabcolsep}{3pt}
            \begin{tabular}{cc}
                \subfloat{\includegraphics[width=0.35\columnwidth]{fig/scene_poly_arrows.pdf}} &
                \subfloat{\includegraphics[width=0.35\columnwidth]{fig/scene_poly_2color.pdf}} \\
                (a*) $2$-Color&
                (b*) $2$-Color \\
                \subfloat{\includegraphics[width=0.35\columnwidth]{fig/scene_poly_guards.pdf}} &
                \subfloat{\includegraphics[width=0.35\columnwidth]{fig/scene_poly_3color.pdf}}\\
                (c*) $3$-Color&
                (d*) $3$-Color
            \end{tabular}
            \vspace{-5pt}
            \caption{Scenarios for the case of translating polygonal robots. Target positions are not indicated in the figures to avoid unnecessary clutter. (a*) $2$-Color scene; the two groups of robots (upward and downward facing arrows) need to exchange positions.  (b*) $2$-Color scene with rectangular and star-shaped robots; the start and target positions were randomly placed. (c*) $3$-Color scene; the two rhombus-shaped robots, which belong to different groups need to exchange positions, while the star-shaped robots need to return to their start positions. (d*). $3$-Color scene with randomly placed start and target positions. }
            \label{fig:scenarios2}
        \end{figure*}

    \noindent\textbf{Test Scenarios.}
    The scenarios for the case of disc robots are illustrated in Figure~\ref{fig:scenarios} and represent a variety of challenging problems. The unlabeled problem in (a) involves the motion of a large collection of robots.
    Scenarios (b) and (e) describe $2$-color and $4$-color problems comprising a large number of robots as well.
    Although scenarios (c), (d) do not involve as many robots, they are nevertheless challenging. This range of problems demonstrate the work of the various components of the \algkp algorithm. In the first three scenarios the resulting pebble graphs have a low number of connected components due to the low value of $k$ (as in scenario (a)) or high clearance from the obstacles (as in (e)). Therefore, large portions of the resulting paths involve the motions of the robots on paths induced by pebble problems. While the generated graphs in scenarios (c) and (d) have low connectivity, \algkp still performs well---due to the use of the connection generator component.
    Additional scenarios, that demonstrate the performance of the algorithm for the case of translating polygonal robots are illustrated in Figure~\ref{fig:scenarios2}.

    The results of running \algkp for specific parameters are given in Table~\ref{table:res}.
    In addition to the parameters mentioned above, the table contains the values $k$ for the number of colors, $m$ the number of robots in every color and $M$ the total number of robots.
    The running times are given in seconds and represent the overall duration of the preprocessing and query phases, for a single query. We mention that the majority of running time was spent on connection of pebble graphs (using the connection generator), and thus we chose to present only the overall running time.
    The parameters used by \algkp and other algorithms, mentioned later on, were manually optimized over a concrete set.
    A failure was declared when an algorithm was unable to solve a scenario for more than three runs out of five. \vspace{2.5pt}

    \noindent\textbf{Comparison with Other Algorithms.}
    The first part of the comparison involves solely inputs of the fully-colored problem.
    We compare \algkp with the implementation of PRM provided by OOPSMP, which, by our experience, is very efficient.
    This algorithm is designed for solving fully-colored \mrmp problems.
    While OOPSMP required 100 seconds to solve scenario (d), \algkp managed to solve it in 1.9 seconds.
    Scenario (c) proved to be even more challenging for OOPSMP, which failed to solve it, even when was given 5000 seconds of preprocessing time, whereas \algkp solved in 213.7 seconds.

    In order to provide a more informative comparison, we ran both algorithms on scenarios (c),(d), only that now  we increased the difficulty of these scenarios gradually---incrementally introducing the robots, i.e., starting with a single robot and adding the others one by one, as long as OOPSMP succeeded solving the new inputs in reasonable time.
    In this case OOPSMP was able to solve scenario (c) with five robots, while the case of six robots was out of its reach (when given 5000 seconds of preprocessing time). The speedup of \algkp compared to OOPSMP for this new range of scenarios is depicted in Figure~\ref{fig:oopsmp} along with an additional test case (``decoupled-simple''), which is a simpler variant of scenario (c) with some of the obstacles removed and the radius of the robots is decreased. The latter was designed to test the performance of OOPSMP on problems involving a higher number of robots.

    \begin{figure*}[b]
                \centering
                \setlength{\tabcolsep}{1pt}
                \begin{tabular}{cc}
                    \subfloat{\includegraphics[width=0.5\columnwidth]{graphs/graph_oops.pdf}} &
                    \subfloat{\includegraphics[width=0.5\columnwidth]{graphs/graph_kbasic.pdf}}
                \end{tabular}
                \vspace{-15pt}
                \caption{\label{fig:oopsmp}Comparing \algkp with OOPSMP/PRM and KBASIC}
                \rimgafter
        \end{figure*}

    As we are not aware of any other algorithms for the $k$-color problem, we designed a basic algorithm to compare \algkp with.
    This algorithm, which we call \algkb, as a special case of \algkp that samples configurations, instead of pumped configurations, and can be viewed as an extension of PRM for the $k$-color case (for more details, see Section~\ref{sec:complete}. The entire set of scenarios (a)-(e),(a*)-(d*) proved to be too challenging for \algkb, which spent at times more than ten minutes.
    Similarly to the previous comparison we designed a set of simple test scenarios.
    Specifically, scenario (e) was converted into five $k$-color problems for $1\leq k\leq 5$ by partitioning the robots into $k$ groups such that a robot number $i$ was assigned to the group $i\;\text{mod}\;k$. Then, as in the previous comparison, the robots were introduced incrementally.
    Figure~\ref{fig:oopsmp} depicts the speedup of \algkp compared with \algkb for each of the $k$-color problems.
    This shows that \algkp outperforms \algkb in every possible setting, be it a $k$-color, unlabeled or fully-colored problem.



==> sec_future.tex <==
\section{Future Work}\label{sec:future}\rsecafter
    A major question remains whether our algorithm, \algkp, is \emph{probabilistically complete} (see Section~1).
    As it is, \algkp is rather challenging to analyze.
    We are currently working on a simplified version of \algkp, which is probabilistically complete and possesses several other useful properties that we wish to investigate in the near future.





==> sec_intro.tex <==
\section{Introduction}\rsecafter
    \emph{Motion planning} is a fundamental problem in robotics and has applications in different fields such as the study of protein folding, computer graphics, computer-aided design and manufacturing (CAD/CAM), and computer games.

    The problem of motion planning, in its most basic form, is to find a collision-free path for a robot from start to goal placements while moving in an environment cluttered with obstacles.

    An obvious extension of this problem is \emph{multi-robot motion planning}, where several robots share a workspace and have to avoid collision with obstacles as well as with fellow robots. In many situations it is natural to assume that some robots are identical, in form and in functionality, and therefore are indistinguishable. In this setting every target position should be occupied by some robot of a kind (and not necessarily by a specific robot). \begin{wrapfigure}{r}{0.4\textwidth}
    \vspace{-15pt}
  \begin{center}
    \includegraphics[width=0.35\textwidth]{fig/thumb.pdf}
  \end{center}
  \vspace{-10pt}
  \caption{An example of a $3$-color scenario where three different groups of robots occupy the same workspace. The star-shaped robots are required to exchange ``rooms'' with the snake robots while the two puzzle-like robots should return to their start positions in the end of the motion.}
  \vspace{-5pt}
\end{wrapfigure}

    \vspace{-10pt}We consider the problem of \emph{$k$-color multi-robot motion planning}---a simple and natural extension of the multi-robot problem where the robots are partitioned into $k$ groups (colors) such that within each group the robots are interchangeable. Every such group has a set of target positions, of size equal to the number of robots in that group. Every robot is no longer required to move to a specific target, but rather to some target position that is assigned to its group. However, we still require that all the target positions will be covered by the end of the motion of the robots. We term the special case where $k=1$ the \emph{unlabeled multi-robot motion planning} problem.

    As an example consider a fleet of mobile robots operating in a factory that are given the task of cleaning a set of specific locations. The robots are indistinguishable from one another, and therefore any robot can be assigned to any location. Now assume that in addition to the mobile robots, another class of maintenance robots is employed by the factory; again, we consider all the maintenance robots to be of the same kind and interchangeable for the given task. This turns the unlabeled problem into a $k$-color problem, where $k=2$ in this case. From now on we will refer to the classic multi-robot motion planning problem as \emph{fully-colored}, as it is a special case of the $k$-color problem where $k$ is equal to the number of robots and every group is of size one.
\rsubbefore
    \subsection{Previous Work}\rsubafter
        Throughout this paper we will assume some familiarity with the basic terms in the area of motion planning. For more background on motion planning, see, e.g., \cite{clhbkt-prmp,l-pa}.

        The first efforts in motion planning in general, and the multi-robot case in particular, were aimed towards the design of \emph{complete} algorithms, guaranteed to find a solution when one exists or report that none exists otherwise. Schwartz and Sharir were the first to give \cite{ss-pm3} a complete algorithm for a multi-robot problem, specifically dealing with the case of coordinating disc robots in the plane. The running time of their algorithm is exponential in the number of robots. A work by Hopcroft et al. \cite{hss-cmpmio} presented soon after suggested that in some cases the exponential running time may be unavoidable, showing that even the relatively simple setting of rectangular robots bound in a rectangular region is PSPACE-hard in the number of robots.

        The hardness of the multi-robot problem involving a large number of robots can be attributed to its high number of \emph{degrees of freedom} (or \emph{dofs})---the sum of the dofs of the individual robots. Some efforts were made in the direction of reducing the effective number of dofs. Aronov et al. \cite{avbsv-mpfmr} showed that for systems of two or three robots a path can be constructed, if one exists, where the robots move while maintaining contact, thus reducing the number of dofs by one or two, depending on the number of robots. van den Berg et al. \cite{bslm-cppmr} proposed a general scheme for decomposing a multi-robot problem into a sequence of subproblems, each consists of a subset of robots, where every subproblem can be solved separately and the results can be combined into a solution for the original problem. This method reduces the number of dofs that need to be treated simultaneously from the number of dofs of the entire problem to the number of dofs of the largest subproblem.

        An opposite approach to the complete planners is the \emph{decoupled} approach, trading completeness with efficiency. Decoupled algorithms solve separate subproblems (usually for individual robots) and combine the individual solutions into a global solution. Although this approach can be efficient in some cases, it does not guarantee finding a solution if one exists and usually works only for a restricted set of problems. An example of such an algorithm can be found in the work of van den Berg and Overmars \cite{bo-pmpmr} where every robot is given a priority and for each robot, the motion path is constructed to avoid collision with both static obstacles and lower-priority robots that are considered as moving obstacles. In other works, as in Leroy et al.~\cite{lls-mpcmr}, individual paths are computed and velocity tuning is performed to avoid collision between robots.

        In recent years, the \emph{sampling-based} approach for motion-planning problems has become increasingly popular due to its efficiency, simplicity and the fact that it is applicable to a wide range of problems.
        Unlike the complete planners that explicitly build the \emph{configuration space} of a given problem, the state of all possible configurations of a robot, sampling-based algorithms construct an implicit representation of a robot configuration space by sampling this space for valid robot placements and connecting nearby samples. The connections between samples form a \emph{roadmap} whose vertices describe valid placements for the robot and the edges represent valid paths from one placement to the other. Due to the implicit representation of the configuration space and their simplicity, sampling-based algorithms tend to be much faster than complete planners in practice, and are applicable to problems with a large number of dofs such as the multi-robot problem. Although these algorithms are not complete, many of them are \emph{probabilistically complete}, that is, they are guaranteed to find a solution, if one exists, given sufficient amount of time. Examples of such algorithms are the PRM algorithm~\cite{kslo-prm} by Kavraki et al. and the RRT algorithm~\cite{l-rert} by Kuffner and LaValle. Such algorithms can be easily extended to the multi-robot case by considering the fleet of robots as one large composite robot~\cite{sl-upp}.
        Several tailor-made sampling-based algorithms have been proposed for the multi-robot case~\cite{hh-hmp,so-cppmr}. For more information on sampling-based algorithms see, e.g., ~\cite{l-pa}.

        An abstract form of the multi-robot motion planning problem is the \emph{pebble motion on graphs problem}~\cite{kms-cpmg}. This is a general case of the famous \emph{15-puzzle} where pebbles occupying distinct vertices of a given graph are moved from one set of vertices to another, where the pebbles are bound to move on the edges of the graph. In~\cite{cdp-rgg} an unlabeled version of the pebble problem is discussed, as well as other variants, such as a grid topology of the graph. In~\cite{gh-mcpm} the feasibility of a $k$-color variant of the pebble problem on a general graphs is discussed. We also mention the work \cite{lb-eccmr} where an algorithm is given for a fairly general pebble problem. A recent work by Wagner et al.~\cite{wmc-ppp12} combines their technique for multi-agent pathfinding in discrete environments~\cite{wc-cmpp11} with an implicit representation of the roadmap, presented by \v{S}vestka and Overmars~\cite{so-cppmr}, to yield an efficient algorithm for the fully-colored multi-robot motion planning problem. In the Conclusion section we discuss more remote variants of multi-robot motion planning.

\rsubbefore
    \subsection{Contribution}\rsubafter
        In this paper we present a sampling-based algorithm for the $k$-color problem (for any $k$). This algorithm is aimed to solve the most general cases of this problem and does not make any assumptions regarding the workspace or the structure of the robots.

        Our algorithm for the $k$-color problem---the \algkp algorithm---reduces the $k$-color problem to several discrete pebble problems. Specifically, a sample generated by \algkp represents a local $k$-color problem that is embedded in a variant of the pebble motion problem. Those pebble problems are constructed in a manner that enables the algorithm to transform movements of pebbles into valid motions of the robots. This allows \algkp to generate a wide range of motions and placements for the robots with minimal investigation of the configuration space, thus reducing the dependence of the algorithm on costly geometric tools such as the collision detector.

        As reflected in the experiments reported below for the case of disc robots and polygonal robots translating in the plane, \algkp proves to be efficient, even on challenging scenes, and is able to solve problems involving a large number of robots using a modest number of samples. Interestingly, it performs well even on inputs of the standard (fully-colored) multi-robot problem.

        This algorithm is simple to implement and does not require special geometric components beyond single-robot local planners and single-robot collision detectors.
        We compare the performance of our algorithm with a simplified version of \algkp that can be considered as a variant of the PRM algorithm for the same problem. We note that the latter performs much slower than \algkp and fails to solve even problems that are considered to be simple for \algkp. Moreover, concentrating on the fully-colored case, \algkp outperforms a state-of-the-art implementation of the PRM algorithm. Our discussion will mainly focus on \algup---an algorithm for the unlabeled case, since its extension for the $k$-color case, namely \algkp, is almost straightforward. \begin{comment}We show that, with the help of a few modification, the \algup algorithm, and consequently the \algkp algorithm, is probabilistically complete.\end{comment}
        The experiments though will demonstrate the power of \algkp for various values of $k$.

        The organization of the paper is as follows. In Section~\ref{secPreliminaries} we give formal definitions of the unlabeled and $k$-color problems. In Section~\ref{secPebble} we present a variant of the pebble problem and discuss its properties which will be exploited by our algorithms. In Section~\ref{secUnlabeled} we present \algup. In the following section (Section~\ref{sec:con}) we describe a subroutine that is used by \algup, which we call the \emph{connection generator}.  In Section~\ref{sec:kpump} we describe the changes that are necessary to transform \algup into \algkp. In section~\ref{sec:complete} the completeness of our algorithm is discussed.  We present experimental results for the case of disc robots and polygonal robots moving among polygonal obstacles in the plane in Section~\ref{sec:results} and discuss certain properties of our techniques in Section~\ref{sec:discussion}, as well as further work.


==> sec_kcolor.tex <==
\vspace{-10pt}
\section{The $k$-Color Case}\label{sec:kpump}
    We describe the changes required to transform \algup into \algkp---an algorithm for the $k$-color problem. We stress that the extension to the $k$-color case is straightforward and we provide it here only for the completeness of presentation. \algkp simultaneously samples several pumped configurations---each corresponds to a different color and hence to a different unlabeled problem. The resulting pebble graphs are constructed in a manner that prevents collision between robots of different colors. This calls for the redefinition of the edge planner mechanism (Section 4) as well as other components.

\vspace{-10pt}
    \subsection{Composite Pebble Graphs}
    \vspace{-10pt}
        We begin with several definitions that extend the primitives presented in the description of \algup. Recall that the $k$-color problem $\L$ is defined by $\U_1,\ldots,\U_k$ where each $\U_i=(R_i,S_i,T_i)$ is an unlabeled problem and $|R_i|=m_i$.
        \begin{comment}Let $\dS=\{S_1,\ldots,S_k\}$, $\dT=\{T_1,\ldots,T_k\}$, be the \emph{start} and \emph{target} composite configurations, respectively.
        \end{comment}

        \begin{definition}
            Let $\dC=\{C_1,\ldots,C_k\}$ be a collection of $k$ configurations, where $C_i$ is a configuration of $\U_i$. $\dC$ is a \emph{composite configuration} if for every $c\in C_i,c'\in C_j$, where $i\neq j$, it holds that $R_i(c)\cap R_j(c')=\emptyset$.
        \end{definition}

        \begin{definition}
            Let $\dV=\{V_1,\ldots,V_k\}$ be a collection of pumped configurations, where $V_i$ is a pumped configuration for $\U_i$. $\dV$ is a \emph{composite pumped configuration} if every $\dC=\{C_1,\ldots,C_k\}$, such that $|C_i|=m_i$ and $C_i\subset V_i$, is a composite configuration.
        \end{definition}

        Let $\dV$ be a composite pumped configuration, as defined above. We construct a pebble graph for every pumped configuration $V_i$ of $\dV$. The edges of every graph are generated in a similar manner to the unlabeled case, although here we impose more restrictions to avoid the collision between robots of different colors.

        Next, we generate the \emph{composite pebble graph} $\dG=\{G_1,\ldots,G_k\}$, where $G_i$ is the pebble graph that resulted from the pumped configuration $V_i$. See an illustration in Figure~\ref{fig:composite_graph}. We now define an equivalence relation between composite configurations of the same composite pebble graph. Recall that two configurations are equivalent, if their signatures are identical (Definition~\ref{def:equiv}). We generalize this notion for the case of composite configurations.
        \begin{figure*}[b]%[!htp]
    \rimgbefore
            \centering
            \setlength{\tabcolsep}{3pt}
            \includegraphics[width=0.5\columnwidth]{fig/kcolor_graph.pdf}
            \vspace{-5pt}
            \caption{An illustration of a composite pebble graph for a 3-color problem, where each group consists of robots of a different shape (square, disc and cross). Note that the positions of the robots are non-overlapping and that robots moving along edges do not collide with stationary robots from the same group or from a different color. }
            \label{fig:composite_graph}
        \end{figure*}
\vspace{5pt}


        \begin{definition}
            Let $\dG=\{G_1,\ldots,G_k\}$ be a composite pebble graph, where $G_i=(V_i,E_i)$. Let $\dC=\{C_1,\ldots,C_k\}, \dC'=\{C'_1,\ldots,C'_k\}$ be two composite configurations, where $C_i,C'_i\subset V_i$. We say that $\dC$ and $\dC'$ are \emph{equivalent}, and denote this relation by $\dC\equiv \dC'$, if for every $1\leq i\leq k$ it holds that $C_i\equiv C'_i$, where the latter ``$\equiv$'' symbol represents the equivalence relation between configurations.
        \end{definition}

        The following proposition is a generalization of Proposition~\ref{thm:gg_path} and its proof is omitted as it is similar to the proof for the unlabeled case.

        \begin{proposition}\label{thm:composite}
            Let $\dC=\{C_1,\ldots,C_k\}, \dC'=\{C'_1,\ldots,C'_k\}$ be two composite configurations of the same composite pebble graph. If $\dC\equiv \dC'$ then there exists a solution to the $k$-color problem $\{\U'_1,\ldots,\U'_k\}$, where $\U'_i=(R_i,C_i,C'_i)$.
        \end{proposition}
\vspace{-10pt}
    \subsection{Description of \Balgkp}
        \vspace{-10pt}
        We describe the sampling-based algorithm for the $k$-color case. \algkp constructs a roadmap $\H$ whose vertices are composite configurations (recall that in \algup, the vertices of this roadmap were configurations). The edges of $\H$ represent valid paths between composite configurations. These paths either connect equivalent composite configurations, as described in Proposition~\ref{thm:composite}, or composite configurations from different composite graphs, where the latter paths are generated using the following mechanism, which is a generalization of the connection generator (Section~\ref{subsec:connect}). Given two composite pumped configurations, and an integer $q$, the  \emph{composite connection generator} returns a collection of $q$ paths, for the $k$-color problem, between the two composite pumped configurations.

        We now return to the description of \algkp. \algkp samples composite pumped configurations $\dV_1,\dV_2,\ldots,\dV_g$ and generates the respective composite pebble graphs $\dG_1,\ldots,\dG_g$. Given a path between two composite configurations $\dC,\dC'$ returned by the composite connection generator we add the vertices $\dC,\dC'$ to $\mathcal{H}$ and the respective edge. Finally we connect the start and target composite configurations $\dS,\dT$, respectively, to previously sampled composite pebble graphs.

        We note that for the fully-colored case these structures remain the same, although the planning on the pebble graphs is simplified a bit since every pebble graph accommodates in this case only a single pebble.


==> sec_pebble.tex <==
\section{The Pebble Motion Problem}\label{secPebble}\rsecafter
    In preparation for the algorithm presented in the next section, we discuss a variant of the problem of \emph{pebble motion on graphs}. This problem is a discretization of the unlabeled problem. This discretization is defined in a manner that will allow us to transform local unlabeled problems into pebble problems such that a movement of the pebbles can be transformed back into valid robot motions. We explain below where our formulation is different from the standard presentation of the pebble-motion problem.

    \subsection{Formal Definition}
        A pebble problem~\cite{kms-cpmg} $\P(G,S,T,m)$ is defined by an undirected graph $G=(V,E)$, and two sets of vertices $S,T\subseteq V$, where $|S|=|T|=m$.
        A \emph{pebble placement} is an ordered set of $m$ distinct vertices of $V$.
        Initially, $m$ identical pebbles $\tau_1,\ldots,\tau_m$ are placed in $S$.
        We wish to find a chain of placements $\pi^*=P_1,\ldots,P_{\ell}$, called a \emph{pebble path}, which obeys the following set of rules. Firstly, we demand that $P_1 = S$.
        Secondly, for every two consecutive placements $P=\{p_1,\ldots,p_m\}, P'=\{p'_1,\ldots,p'_m\}$ and every $1\leq i \leq m$ it holds that $(p_i,p'_i)\in E$ or $p_i = p'_i$, \ie, the pebble $\tau_i$ is allowed to stay in its current vertex or move to a neighboring vertex in the graph.

        Next we depart from the problem definition in~\cite{kms-cpmg}. We demand that $P_{\ell}$ is some permutation of the elements of $T$. (The original formulation~\cite{kms-cpmg} specified which pebble will reside on which specific vertex of $T$.) We do, however, impose an additional requirement---the \emph{separation rule}---which requires that the pebbles will move separately, \ie, for every two consecutive placements $P,P'$, as defined above, exactly one pebble $\tau_i$ makes a move on an edge, while the other pebbles remain stationary. More formally, there exists $1\leq i\leq m$ such that $(p_i,p'_i)\in E$ and for every $j\neq i$ it holds that $p_j=p'_j$. The reason for this restriction will become clear later on.

    \subsection{Solvability}
        We provide a simple test to identify whether a given pebble problem has a solution. We start with a pair of basic definitions.

        \begin{definition}%[Signature]
            Let $V'$ be a pebble placement of a pebble problem $\P(G,S,T,m)$ and let $\{G_1,\ldots,G_h\}$ be the set of maximal connected subgraphs of $G$, where $G_i=(V_i,E_i)$. The \emph{signature} of $V'$ is defined as $\sig(G,V')=\{|V'\cap V_i|\}_{i=1}^h$.
        \end{definition}
        Namely, the signature of a placement is the number of pebbles in every connected component. Using this definition we define an equivalence relation between placements.

        \begin{definition}\label{def:equiv}%[Equivalence of Placements]
            Let $V',V''$ be two placements of $\P(G,S,T,m)$. We say that the two placements are equivalent if $\sig(G,V')=\sig(G,V'')$ and denote this property by $V'\equiv V''$.
        \end{definition}

        We note that this equivalence relation is defined between placements of the same graph. The variant of the pebble problem used in this paper possesses the following property, which states that there exists a pebble path between every two equivalent pebble placements. This property plays a cental role in the design of the \algup algorithm, presented in the next sections.
        \begin{lemma}\label{lem:pebble_property}\rlembefore
            For every pebble problem $\P(G,S,T,m)$ such that $S\equiv T$, there exists a pebble path from $S$ to $T$.
        \end{lemma}

        This lemma is a generalization of ~\cite[Section 3, first Lemma]{k-cpmg} where an algorithm for the case of a connected graph is given. We mention that this algorithm constructs a spanning tree of $G$ and restricts the movements of the pebbles to the edges of the tree.

        From now on, we will refer to the algorithm that solves the pebble problem as \emph{pebble solver}, which given a pebble problem returns a pebble path.

        \begin{comment}From now on, we will refer to this algorithm as \emph{pebble solver}.
        We mention that it produces paths of length $O(n^2)$, and although is not necessarily optimal (since a path in $G$ can be much shorter than the path in $\T$) such number of moves is sometimes required. For example, consider a graph $G$ that consists of a single chain of vertices and the pebble residing in one side of the chain are required to move to the other side where the number of pebbles is half of the number of vertices.\end{comment}



        \begin{comment}Although the running time of this algorithm is not discussed in \cite{k-cpmg}, a simple approach where the closest occupied (or unoccupied) vertex is found using a BFS algorithm, will yield a running time of $O(n^2)$. \end{comment}


==> sec_pebble_solver.tex <==
\section{Pebble Problem Solver}
    \begin{comment}
        We describe a simple algorithm for solving the pebble problem described in the main paper.
        Recall that the problem consists of a graph $G=(V,E)$ and two pebble placements $S,T$ where $|S|=|T|=m$.
        For simplicity we will assume that $G$ is composed of a single connected component.
        The pebble solver constructs a spanning tree $H$ of the graph $G$ and places the $m$ pebbles $\tau_1,\ldots,\tau_m$ on the nodes $S$ of $H$.

        In the first step the solver \emph{lowers} all the pebbles to the bottom of the tree. Formally, by the end of the process the pebble are either situated in the leaves of $H$ or in vertices all whose subtrees are full with pebbles.

        In the next step the solver \emph{balances} the pebbles in $H$ such that in at the end of this step every subtree of $H$ that is connected to the root will contain the same number of pebbles as it would have contained if the pebbles were placed on $T$.  Suppose that the root of $H$, $v_{root}$, has $\ell$ children and let $H_1,\ldots,H_\ell$ be the subtrees that are connected to $v_{root}$. Denote by $\alpha_i$ the number of pebbles that are currently placed in $H_i$. Similarly, $\beta_i$ denotes the number of pebbles from the placement $T$ that are placed in $H_i$, i.e., $\beta_i = |V_i\cap T|$ where $V_i$ denotes the set of vertices of $H_i$. In addition, let $\gamma_i = \alpha_i - \beta_i$.

        For every subtree $H_i$ such that $\gamma_i<0$ the solver transfers $-\gamma_i$ pebbles, one by one, from other trees to $H_i$. For every ``missing'' pebble of $H_i$ the solver selects a tree $H_j$ for which $\gamma_j>0$. The topmost pebble of $H_j$ is selected, i.e., a pebble which is the closest to the root of $H_j$. This pebble is moved to the top of the tree $H_j$, then, through $v_{root}$, moved to the subtree $H_i$. When this pebble reaches $H_i$ it is lowered to a vacant leaf of $H_i$ or to a vacant vertex such that all the subtrees connected to it are full with pebbles. Once this operation is complete we update the values of $\gamma_i,\gamma_j$---increment $\gamma_i$ and decrement $\gamma_j$. This operation is repeated until $\gamma_i=0$ for $H_i$ and for every other $H_{i'}$ such that $\gamma_{i'}<0$. If we end up with one subtree $H_j$ for which $\gamma_j=1$ (while the other subtrees are balanced) we move one last pebble from $H_j$ to $v_{root}$. The latter situation occurs when $v_{root}\in T$.

        Finally, we recursively apply the \emph{balance} step on every subtree $H_i$ . We mention that all the movements of the pebbles are recorded.

        We chose not to discuss the running time of this solver in this paper as its effect on the total running time of \algkp is negligible.
    \end{comment}

    A simple algorithm for the unlabeled case of the pebble problem is given by Kornhauser~\cite[Section 3, first Lemma]{k-cpmg}. For the sake of completeness we briefly describe this algorithm. Let $\P(G)$ be a pebble problem where $G=(V,E)$ and suppose that $S,T$ are pebble placements such that $|S|=|T|=k$. The pebble solver constructs a spanning tree $\T$ of $G$ and places the pebbles on the vertices $S$ of $\T$.

    The solver selects some vertex $v$ that is a leaf of $\T$. If $v\in T$ then this vertex should be occupied with a pebble. If this vertex is already occupied the treatment of this vertex is completed. Otherwise, the solver finds the closest pebble to $v$ in $\T$ and moves this pebble to the leaf. Since it is the closest pebble we can freely move the pebble without moving other pebbles.

    On the other hand, if $v\not\in T$ then a pebble residing in $v$ should be evacuated. To achieve this goal the solver finds the closest unoccupied vertex $v'$ to $v$ of $\T$ and ``pushes'' the pebbles on this shortest path towards $v'$, one by one, until $v$ is no longer occupied.

    Once the treatment of $v$ has completed we remove this leaf from the tree, i.e., $\T\leftarrow \T\setminus\{v\}$, and select another leaf of $\T$ to be treated. The solver terminates when $\T$ is composed of a single vertex.
    
    This algorithm produces paths of length $O(n^2)$ and although is not necessarily optimal (since the path in $G$ can be much shorter than the path in $\T$) such number of moves is sometimes required. For example, consider a graph $G$ that is composed of a chain of vertices and the pebble residing in one side of the chain are required to move to the other side where the number of pebbles is half of the number of vertices. Although the running time of this algorithm is not discussed in \cite{k-cpmg}, a simple approach where the closest occupied (or unoccupied) vertex is found using a BFS algorithm, will yield a running time of $O(n^2)$.



==> sec_prel.tex <==
\section{Preliminaries and Terminology} \label{secPreliminaries}\rsecafter
    Let $r$ be a robot operating in the workspace $W$. We denote by $\F(r)$ the \emph{free space} of a robot $r$---the collection of all collision-free \emph{\sr configurations}.\footnote{We assume that $\F(r)$ is an open set. This is not critical in the algorithms below as we assume that
the robot never moves in contact with the obstacles.} Given $s,t\in \mathcal{F}(r)$, a \emph{path} for $r$ from $s$ to $t$ is a continuous function $\pi:[0,1]\rightarrow \mathcal{F}(r)$, such that $\pi(0)=s, \pi(1)=t$.\vspace{5pt}

    \noindent\textbf{Unlabeled Multi-Robot Motion Planning.}
        We say that two robots $r,r'$ are \emph{geometrically identical} if $\F(r) = \F(r')$ for the same workspace $W$. Let $R=\{r_1,\ldots,r_m\}$ be a set of $m$ geometrically identical robots, operating in a workspace $W$. We may use $\mathcal{F}$ to denote $\mathcal{F}(r_i)$ for any $1\leq i \leq m$. Let $C=\{c_1,\ldots,c_m|c_i\in \F\}$ be a set of $m$ single-robot configurations. $C$ is a \emph{configuration} if for every $c,c'\in C$, with $c\neq c'$, the robots $r,r'\in R$, placed in $c,c'$, do not collide.
        Notice that we reserve the unqualified term \emph{configuration} to refer to a set of $m$ collision-free single-robot configurations. Other types of configurations will be qualified: single-robot configurations and pumped configurations.

        Given two configurations $S=\{s_1,\ldots,s_m\},T=\{t_1,\ldots,t_m\}$, named \emph{start} and \emph{target}, respectively, we define $\mathcal{U}=(R,S,T)$ as the \emph{unlabeled problem}, which is shorthand for the {\it unlabeled multi-robot motion planning problem}. Our goal is to find an \emph{unlabeled path} $\pi_{\mathcal{U}}$, defined as follows. Firstly, $\pi_{\mathcal{U}}$ is a collection of $m$ paths $\{\pi_{1},\ldots,\pi_{m}\}$ such that for every $i$, $\pi_{i}$ is a collision-free path for the robot $r_i$ from $s_i$ to {\it some} $t\in T$. Secondly, the robots have to remain collision-free while moving on the respective paths, i.e., for every $\theta \in [0,1]$, $\pi_{\U}(\theta)=\{\pi_{1}(\theta),\ldots,\pi_{m}(\theta)\}$ is a configuration. Notice that this also implies that $\pi_{\U}(1)$ is some permutation of $T$.

        Throughout this paper, we use the notation $r(c)\subset\C$, for $c\in \F$, to represent the portion of the configuration space covered by a robot $r\in R$ placed in the \sr configuration $c$. Note that two robots from $R$ collide, when placed in $c,c'\in \F$, if $r(c)\cap r(c')\neq \emptyset$.
    \vspace{5pt}

    \noindent\textbf{$k$-Color Multi-Robot Motion Planning.}
        The $k$-color problem $\mathcal{L}$ is defined by the set of unlabeled problems $\{\mathcal{U}_1,\ldots,\mathcal{U}_k\}$, where $\U_i=(R_i,S_i,T_i)$ and $|R_i|=m_i$. The definition of the solution to this problem, namely a \emph{$k$-color path}, immediately follows. A special case of this problem, usually named simply \emph{multi-robot motion planning}, is a $k$-color problem where for every $\mathcal{U}_i$ it holds that $|R_i|=1$. In our context we call this special case \emph{fully-colored}.


==> sec_unlabeled_pumping.tex <==
\section{The Unlabeled Case: Pumped Configurations} \label{secUnlabeled}\rsecafter
    In this section, we present our main contribution --- a sampling-based algorithm for the unlabeled problem. At a high level the \algup algorithm bears some resemblance to the PRM algorithm, as they both generate a collection of samples that form a roadmap. However, the structures and subroutines used by \algup are quite different from the ones used by PRM. Thus, we describe \algup independently from PRM.

    \algup generates a collection of geometrically-embedded graphs. These are called \emph{pebble graphs} and enable the mapping of valid movements of pebbles from one pebble placement to the other on these graphs, into motions of robots between configurations. The vertices of such pebble graphs are \sr configurations while the edges represent \sr paths. We generate a pebble graph by sampling a set of single-robot configurations, called \emph{pumped configurations}, of size larger than the actual number of robots, to seemingly accommodate an increased number of robots.

    This technique makes use of the fact that our problem does not involve one complex robot, but rather a collection of robots operating in the same configuration space. This is in contrast with a popular \sbs technique that considers the group of robots as one \emph{composite robot}. In our opinion, the latter suffers from an acute disadvantage compared to our technique. We will demonstrate this claim experimentally and discuss the benefits of \algup and \algkp in depth later on.

    After discussing the construction of pebble graphs and exploring their various properties we show that they can be connected to generate more complex paths where the robots not only move within a single pebble graph but also between different pebble graphs on collision-free paths. We conclude this section with a description of the sampling-based algorithm.

\rsubbefore
    \subsection{Construction of Pebble Graphs}
    \label{subsec:constrion_pebble}\rsubafter
        We now define more formally some of the aforementioned structures. Recall that a configuration is a collection of $m$ \sr configurations, where $m$ is the actual number of robots, i.e., $|R|=m$, for which the $m$ robots are collision-free.

        \rlembefore\begin{definition}%[Pumped Configuration]%
            Let $V=\{v_1,\ldots,v_{n}\}$ for $n\geq m$ be a set of single-robot configurations such that for every $v\in V$ it holds that $v\in \F$, where $\F=\F(r)$ for some $r\in R$. $V$ is a \emph{pumped configuration} if for every $v,v'\in V$ two robots placed in these \sr configurations do not collide.
        \end{definition}\rlemafter

        Note that this implies that every subset of size $m$ of a pumped configuration is a configuration, i.e., if $C\subset V, |C|=m$ then $C$ is a configuration. Additionally, it follows that a pumped configuration can accommodate an increased number of robots, $n$ to be exact. A possible implementation of a procedure that generates a pumped configuration is given in Algorithm~\ref{alg:pumped_configuration}.

        Given a pumped configuration $V$ we construct the graph $G=(V,E)$ where the edges represent paths in $\F$ for individual robots. We call it a \emph{pebble graph}, and view it as embedded in the free configuration space. To generate the edges of $G$, and the respective paths, we utilize the \emph{edge planner} mechanism that is described below. This, in turn, relies on the \emph{local planner} component, that traditionally attempts to connect two \sr configurations with a straight-line path, although a more sophisticated technique can be used.

        Let $v,v'\in V$ be two distinct \sr configurations of the pumped configuration $V$, and let $\pi$ be a path for $r\in R$ from $v$ to $v'$ that was generated by the local planner. If for every $u\in V$, where $u\neq v,v'$, the robot $r$, while moving on $\pi$, does not collide with a (geometrically identical) robot placed in $u$, then the \emph{edge planner} returns $\pi$. Otherwise, it reports failure. Thus, the edge planner returns only paths for which a robot moving between two \sr configurations does not collide with other stationary robots placed in other \sr configuration of $V$.

        To construct a pebble graph from a pumped configuration $V$, the edge planner is applied on every pair $v\neq v'$ in $V$. Upon successful generation of a path $\pi_{v,v'}$ the edge $(v,v')$ is added to $G$. An example of a pumped configuration, as well as its underlying graph, are given in Figure~\ref{fig:cs}. A formal definition of the pebble graph is given constructively in Algorithm~\ref{alg:geometric_graph}.

        \begin{figure}[th]
            \vspace{-10pt}
            \rimgbefore
            \centering
            \setlength{\tabcolsep}{3pt}
            \begin{tabular}{cc}
                \subfloat{\includegraphics[width=0.35\columnwidth]{fig/CS1.pdf}} &
                \subfloat{\includegraphics[width=0.35\columnwidth]{fig/CS2.pdf}} \\
                (a)&(b)
            \end{tabular}
            \vspace{-5pt}
            \caption{(a) Pumped configuration $V$ with $m=3, n=7$, for the problem of disc robots in the plane. $C,C'$ are two configurations such that $C,C'\subset V$. (b) The pebble graph $G$ is induced by $V$ using an edge planner that tries to connect pairs of \sr configurations with a straight-line path. In addition, a path induced by a pebble path, from $C$ to $C'$, is described, where the arrows describe the movements of the robots from one single-robot configuration to its neighbor, and the numbers indicate the order in which those movements occur.}
            \label{fig:cs}
            %\rimgafter
        \end{figure}

        \begin{algorithm}[!ht]
            \caption{PUMPED\_CONFIGURATION($n$)}
            \label{alg:pumped_configuration}
            \begin{algorithmic}[1]
                        \STATE  $V\leftarrow\emptyset$
                        \WHILE  {$|V|\not =n$}
                            \STATE  $v\leftarrow$ RANDOM\_SAMPLE()
                            \STATE  $\text{valid}\leftarrow\text{TRUE}$
                            \FORALL  {$v'\in V,\; v\neq v'$}
                                \IF {$r(v)\cap r(v')\neq \emptyset$}
                                    \STATE $\text{valid} \leftarrow \text{FALSE}$
                                \ENDIF
                            \ENDFOR
                            \IF {valid}
                                \STATE $V\leftarrow V\cup\{v\}$
                            \ENDIF
                        \ENDWHILE
                        \RETURN $V$
            \end{algorithmic}
        \end{algorithm}

        \begin{algorithm}[!ht]
            \caption{PEBBLE\_GRAPH($n$)}
            \label{alg:geometric_graph}
            \begin{algorithmic}[1]
                \STATE  $V\leftarrow$ PUMPED\_CONFIGURATION($n$)
                \STATE  $E\leftarrow \emptyset$
                \FORALL {$v,v'\in V,\; v\neq v'$}
                        \STATE $\pi_{v,v'}\leftarrow \text{EDGE\_PLANNER}(V,v,v')$
                        \IF {$\pi_{v,v'}\not = \bot$}
                            \STATE $E\leftarrow E\cup \{(v,v')\}$
                        \ENDIF
                \ENDFOR
                \RETURN $G=(V,E)$
            \end{algorithmic}
        \end{algorithm}

    \subsection{Properties of Pebble Graphs}
        We now discuss the various properties of this special graph. We first note that every configuration $C\subset V$ is also a pebble placement for some pebble problem that is defined on $G$. A less obvious property of the pebble graph $G$, which is described in the following proposition, allows us to transform pebble paths into robot paths.

        \begin{proposition}\label{thm:gg_path}
            Let $G=(V,E)$ be a pebble graph and let $C,C'\subset V$ be two configurations such that $C\equiv C'$. Then there exists a path $\pi_{\U'}$ for $\U'=(C,C')$.
        \end{proposition}
        \begin{proof}
            By Lemma~\ref{lem:pebble_property} there is a pebble path $\pi^*$ for the pebble problem $\P(G,C,C',m)$. We transform the movements of the pebbles into $\pi^*$ to a valid motion of the robots in the following manner.
            A movement of the pebble $\tau_i$ on the edge $(v,v')\in E$ is transformed to the motion of the robot $r_i$ along the path $\pi_{v,v'}$. Notice that a collision between a robot and an obstacle cannot occur since the path was generated by the edge planner. Additionally, a moving robot cannot collide with another ``stationary'' robot that resides in some other vertex $u\in V$. Finally, a collision between two moving robots cannot occur since the pebble path $\pi^*$ must respect the separation rule (Section~\ref{secPebble}), which states that at most one pebble is allowed to move at a given time. \qed
        \end{proof}

\rsubbefore
    \subsection{Connecting Pebble Graphs}\label{subsec:connect}\rsubafter
        Proposition~\ref{thm:gg_path} implies that certain unlabeled problems can be solved using a single pebble graph. However, this statement does not hold for many other instances of the unlabeled problem. As an example, consider an unlabeled problem $\U=(S,T)$ in which there exists at least one pair $s\in S, t\in T, s\neq t$, such that a robot $r\in R$ placed in $s$ overlaps with another robot $r'\in R$ placed in $t$. Thus, $s,t$ cannot be in the same pumped configuration.

        Fortunately, we can combine several graphs in order to find paths for more general unlabeled problems. For instance, robots may move from a pebble graph $G_S=(V,E)$ where $S\subset V$, through several other pebble graphs until they will finally reach $G_T=(V',E')$ where $T\subset V'$.

        We first show that given two pebble graphs and an unlabeled path connecting two configurations, one from every graph, the robots can move from the first pebble graph to the second. This path serves as a ``bridge'' between the two graphs and connects not only the two configurations but many other configurations from the two graphs as well. Before describing a mechanism to generate such paths we provide a concrete description of the property discussed here in the form of the following lemma. We omit its proof, which is straightforward.\begin{figure*}[b]%[!htp]
    \rimgbefore
            \centering
            \setlength{\tabcolsep}{3pt}
            \begin{tabular}{ccc}
                \subfloat{\includegraphics[width=0.3\columnwidth]{fig/path1a.pdf}} &
                \subfloat{\includegraphics[width=0.3\columnwidth]{fig/path1b.pdf}} &
                \subfloat{\includegraphics[width=0.3\columnwidth]{fig/path2.pdf}}\\
                (a) &
                (b) &
                (c)
            \end{tabular}
            \begin{tabular}{cc}
                \subfloat{\includegraphics[width=0.3\columnwidth]{fig/path3a.pdf}} &
                \subfloat{\includegraphics[width=0.3\columnwidth]{fig/path3b.pdf}}\\
                (d) &
                (e)
            \end{tabular}
            \vspace{-5pt}
            \caption{An illustration of a path between two pebble graphs, as described in Lemma~\ref{lem:connecting_ggs}, from a configuration $D$ of the pebble graph $G$, to a configuration $D'$ of $G'$. $G$ consists of five vertices and two connected components, as illustrated in (a),(b), and $G'$ consists of four vertices with two connected components, as shown in (d),(e). In (a) the starting configuration $D$ of the two robots is shown. In (b) the robots move according to a pebble-induced path to the configuration $C$. In (c) the robots move from $G$ to $G'$ by a path that connects $C$ with $C'$. In (d) and (e) the two robots move from $C'$ to $D'$ according to a pebble induced path on $G'$. Notice that $C\equiv C', D\equiv D'$, as required.}
            \label{fig:graph_connection}
        \end{figure*}
\vspace{5pt}

        \begin{lemma}\rlembefore\label{lem:connecting_ggs}
            Let $C\subset V,C'\subset V'$ be two configurations of the pebble graphs $G=(V,E),G'=(V',E')$ and let $\pi_{C,C'}$ be a path for the unlabeled problem $\U'=(C,C')$. In addition, let $D,D'$ be two configurations such that $D\subset V, D'\subset V'$ and $D\equiv C, D'\equiv C'$. Then there exists a path $\pi_{\U''}$ for $\U''=(D,D')$.
        \end{lemma}\rlemafter

       An example of a path, as described in Lemma~\ref{lem:connecting_ggs}, is given in Figure~\ref{fig:graph_connection}. Paths similar to $\pi_{C,C'}$ described above are generated using the following component which generalizes the component \emph{local planner} used in standard \sbs algorithms. We postpone a detailed description of this component to Section~\ref{sec:con}.

        Given two pumped configurations $V,V'$ the \emph{connection generator} returns $q$ several paths such that every returned path $\pi_{C,C'}$ is a solution for some unlabeled problem $\U'=(C,C')$ where $C,C'$ are configurations such that $C\subset V, C'\subset V'$.

        By Lemma~\ref{lem:connecting_ggs}, a single connection implicitly connects a collection of configurations with a specific signature from the first graph with a similar collection in the second graph. We require from the connection generator to create several such connections in order to connect a variety of signatures between the two graphs.
\rsubbefore
    \subsection{Description of \Balgup}\rsubafter
        Next, we extend Lemma~\ref{lem:connecting_ggs} to describe still more complex paths. The \algup algorithm has a preprocessing phase and a query phase. In the first phase it samples a collection of pebble graphs and connects them using the \congen. Those connections represent edges in a roadmap $\H$ whose vertices are configurations from the different pebble graphs. Additional edges, that represent paths between configurations within the same pebble graph, are added to $\H$ afterwards. In the query phase, given start and target configurations $S,T$, \algup generates two pebble graphs that contain them. These two graphs are connected to other previously sampled pebble graphs. We give a more formal description below, along with the description of the parameters used by \algup.\vspace{5pt}

        \noindent\textbf{Parameters.} $g$ is the number of sampled pebble graphs; $n$ represents the size of a sampled pumped configuration; $q$ is the maximal number of connections between two pebble graphs.\vspace{5pt}

        \noindent\textbf{Preprocessing (Algorithm~\ref{alg:preprocess}).} \algup samples a collection of $g$ pebble graphs $\G$ (line 3). For every pair of sampled pebble graphs $G=(V,E),G'=(V',E')$ we apply the CONNECT procedure (line 6)  that generates several connections between the two pebble graphs, and updates the roadmap accordingly. Then, we add edges to $\H$ that represent connections that follow from Proposition~\ref{thm:gg_path} (line 8). We remind the reader that two configurations are equivalent only if they were taken from the same pebble graph, and their signatures are identical. We draw an edge between them but do not generate the respective paths at this point, as only some of them will eventually participate in a path returned in the query phase (an economical ``lazy'' approach) \textbf{This concept is further discussed in the paragraph describing the path retrieval stage below}.\vspace{5pt}


        \begin{algorithm}[bh!]
            \caption{PREPROCESS($g,q,n$)}
            \label{alg:preprocess}
            \begin{algorithmic}[1]
                \STATE  $\V\leftarrow \emptyset;\; \E\leftarrow \emptyset;\;\H=(\V,\E)$
                \STATE  $\G\leftarrow \emptyset$
                \FOR{$i = 1 \to g$}
                    \STATE  $G\leftarrow$ PEBBLE\_GRAPH($n$)
                    \STATE  $\G\leftarrow \G\cup \{G\}$
                \ENDFOR
                \FORALL {$G,G'\in \G$}
                    \STATE CONNECT($G,G',\H,q$)
                \ENDFOR
                \FORALL {$C,C'\in \V$ where $C\equiv C'$}
                    \STATE $\E\leftarrow \E\cup\{(C,C')\}$
                \ENDFOR
            \end{algorithmic}
        \end{algorithm}

        \noindent\textbf{Connect (Algorithm~\ref{alg:connect}).}
        This is an auxiliary method that uses the \congen component to connect two given pebble graphs (line 1). For every path $\pi_{C,C'}$ returned by the  \congen, where $C,C'$ are configurations of $G,G'$, respectively, $C$ and $C'$ are added as vertices to the roadmap $\H$ together with an edge between them. As this edge may be used later on as a part of a path for the robots, we attach to it the actual path $\pi_{C,C'}$, which was generated by the \congen.\vspace{5pt}

        \begin{algorithm}[bh!]
            \caption{CONNECT($G=(V,E),G'=(V',E'),\H=(\V,\E),q$)}
            \label{alg:connect}
            \begin{algorithmic}[1]
                \STATE $\{(C_1,C'_1),\ldots, (C_q,C'_q)\} \leftarrow \text{CONGEN}(V,V',q)$
                \FOR {$i=1\to q$}
                    \STATE $\V\leftarrow \V\cup\{C_i,C'_i\}$
                    \STATE $\E\leftarrow \E\cup\{(C_i,C'_i)\}$
                \ENDFOR
            \end{algorithmic}
        \end{algorithm}

        \noindent\textbf{Query (Algorithm~\ref{alg:query}).} In this phase, \algup is given the start and target configurations. As $S,T$ can be considered as pumped configurations (containing $m$ \sr configurations) we generate the respective pebble graphs $G_S,G_T$ (line 1). We then connect $G_S,G_T$ to previously sampled pebble graphs using the \congen and add relevant vertices and edges to $\H$ (CONNECT procedure described in Algorithm~\ref{alg:connect}). Finally, if $S,T$ are connected in $\H$ a path retrieval is carried out. \vspace{5pt}

         \begin{algorithm}[bh!]
            \caption{QUERY($S,T,q$)}
            \label{alg:query}
            \begin{algorithmic}[1]
                \STATE $G_S=(S,\emptyset)$; $G_T=(T,\emptyset)$
                \FORALL {$G\in \G$}
                    \STATE CONNECT($G,G_S,\H,q$)
                    \STATE CONNECT($G,G_T,\H,q$)
                \ENDFOR
                \IF {$S,T$ not connected in $\H$}
                    \RETURN FAILURE
                \ENDIF
                \RETURN RETRIEVE\_PATH($\H,S,T$)
            \end{algorithmic}
        \end{algorithm}

        \noindent\textbf{Path Retrieval (Algorithm~\ref{alg:retrieve}).}
        Using a graph search algorithm, a path is found between $S$ and $T$ in $\H$ (line 2). Then, it is transformed into a solution to the unlabeled problem $\U=(R,S,T)$. If two consecutive configurations $C_{i-1},C_{i}$ on the path are equivalent, then the respective pebble path is produced (line 6) and converted to a path for the unlabeled problem $\U=(R,C_{i-1},C_i)$, following the process described in Proposition~\ref{thm:gg_path}. If on the other hand $C_{i-1}\not\equiv C_{i}$, then the path $\pi_{C_{i-1},C_i}$, that was generated by the \congen, is used.

        Notice that while $\H$ may contain many equivalent configurations that share an edge in $\H$, the actual paths between such configurations (that are induced by pebble problems) are only generated if these configurations appear on a path that is found in the retrieval stage.

        \begin{algorithm}[bt!]
            \caption{RETRIEVE\_PATH($\H,S,T$)}
            \label{alg:retrieve}
            \begin{algorithmic}[1]
                \STATE $\Pi\leftarrow \emptyset$
                \STATE $\{C_0,\ldots,C_\ell\}\leftarrow \text{GRAPH\_PATH}(\H,S,T)$
                \FOR {$i=1\to \ell$}
                    \IF {$C_{i-1}\equiv C_i$}
                        \STATE $G\leftarrow$ pebble graph of $C_i$
                        \STATE $\pi^*\leftarrow \text{PEBBLE\_SOLVER}(G,C_{i-1},C_i)$
                        \STATE $\pi\leftarrow \text{TRANSFORM\_PATH}(\pi^*)$
                        \STATE $\Pi$.append($\pi$)
                    \ELSE
                        \STATE $\Pi$.append($\pi_{C_{i-1},C_{i}}$)
                    \ENDIF
                \ENDFOR
                \RETURN $\Pi$
            \end{algorithmic}
        \end{algorithm}

        \vspace{-10pt} 
